Video Diffusion Avatars: Taming Video Diffusion Models into Controllable 3D Avatars

Video diffusion models (VDMs) trained on internet-scale data encode a rich prior on appearance, motion, and physics that is difficult to replicate with explicit 3D rendering and costly 3D data capture. We introduce Video Diffusion Avatars (VDAs), a method that creates photo-realistic, multi-view consistent avatars from a single image by fine-tuning a VDM for precise control over camera viewpoint, facial expression, and upper-body pose. Departing from 3D morphable models (3DMMs), VDAs use a learned expression space that lifts the expressiveness ceiling of 3DMMs, e.g., for the tongue and mouth interior. However, learned expression codes exhibit heavy viewpoint bias, as our DISTRACT benchmark reveals. We show that this bias can be removed through disentanglement, enabling their use as driving signals for multi-view consistent avatars. Camera and upper-body pose are controlled jointly via proxy-mesh renderings, giving independent control over expression, pose, and viewpoint. A camera-triplet training strategy makes the approach efficient: our models train for 34 hours on a single A100 using only public multi-view data. VDAs outperform state-of-the-art single-image 3D avatars on novel-view reenactment, reducing face LPIPS by 29% and improving perceptual quality (JOD) by 66% on BecomingLit. A static 3DGS reconstruction probe further confirms that our generations are the most multi-view consistent. Built on a video prior, VDAs produce effects beyond the reach of explicit renderers, including physically plausible hair dynamics, shadows, reflections, and refractions.

==> preamble.tex <==

\makeatletter\@ifundefined{ificlr}{\newif\ificlr}{}\makeatother
\providecommand{\vdasuppvideo}{supplementary video}


\ificlr
  \newenvironment{strip}{\par\noindent\begin{minipage}{\linewidth}}{\end{minipage}\par}
\else
  \usepackage{cuted} %
\fi

\usepackage{overpic}
\usepackage{adjustbox} %
\ificlr\newcommand{\tabcite}[1]{}\else\newcommand{\tabcite}[1]{~\cite{#1}}\fi

\newlength{\cparagraphskip}\setlength{\cparagraphskip}{0pt}
\ificlr
  \makeatletter
  \newcommand{\cparagraph}[1]{\par\vspace{\dimexpr\cparagraphskip-\parskip\relax}%
    \def\cparagraph@title{#1}%
    \everypar{\setbox\z@\lastbox\everypar{}\textbf{\cparagraph@title}\hspace{0.5em}}}
  \makeatother
\else
  \newcommand{\cparagraph}[1]{\paragraph{#1}}
\fi

\makeatletter
\newcommand{\iclrnofloats}{%
  \renewenvironment{figure}[1][]{\def\@captype{figure}\centering}{}%
  \renewenvironment{table}[1][]{\def\@captype{table}\centering}{}}
\makeatother

\usepackage{currfile} %

\usepackage{multirow}

\usepackage{placeins}

\usepackage{caption} %

\newif\ifpresentable
\presentabletrue  %

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{\ifpresentable #1\else{\color{red}#1}\fi}
\newcommand{\TODO}[1]{\ifpresentable\else\textbf{\color{red}[TODO: #1]}\fi}
\definecolor{profpurple}{rgb}{0.55,0.0,0.55}
\newcommand{\PROF}[1]{\textbf{\color{profpurple}[PROF: #1]}}

\newcommand{\Placeholder}[3][2.4in]{%
  \ifpresentable
    \fbox{\begin{minipage}[c][#1][c]{0.98\linewidth}\centering\Large\itshape #2\end{minipage}}%
  \else
    \fbox{\begin{minipage}[c][#1][c]{0.98\linewidth}\centering\TODO{#3}\end{minipage}}%
  \fi
}




\usepackage{xspace}
\newcommand{\OURS}{VDAs\xspace}

\DeclareMathAlphabet{\mathnet}{U}{eus}{m}{n}
\newcommand{\net}[1]{\mathnet{#1}}
\newcommand{\zc}[2]{\mathbf{z}^{\text{#1}}_{\text{#2}}}



\ificlr

\fi

\usepackage{colortbl}
\definecolor{tabfirst}{rgb}{1, 0.7, 0.7}
\definecolor{tabsecond}{rgb}{1, 0.85, 0.7}
\definecolor{tabthird}{rgb}{1, 1, 0.7}
\definecolor{txtfirst}{rgb}{0.75, 0, 0}
\definecolor{txtsecond}{rgb}{0.8, 0.42, 0}
\definecolor{txtthird}{rgb}{0.55, 0.48, 0}

\usepackage{tikz}
\usetikzlibrary{positioning, arrows.meta, calc, fit, backgrounds, shapes.geometric}

\definecolor{ptblue}{HTML}{4477AA}
\definecolor{ptcyan}{HTML}{66CCEE}
\definecolor{ptgreen}{HTML}{228833}
\definecolor{ptgrey}{HTML}{BBBBBB}

\definecolor{bgPrimary}{HTML}{E8DAEF}
\definecolor{bgSecondary}{HTML}{D4E6F1}
\definecolor{bgAccent}{HTML}{D2B4DE}
\definecolor{bgInput}{HTML}{F4ECF7}
\definecolor{borderPrimary}{HTML}{AF7AC5}
\definecolor{borderAccent}{HTML}{7D3C98}
\definecolor{arrowColor}{HTML}{6C3483}
\definecolor{textMain}{HTML}{2C2C54}
\definecolor{textLight}{HTML}{7F8FA6}
\definecolor{bgHighlight}{HTML}{FDEBD0}

\tikzset{
  module/.style={
    draw=borderPrimary, fill=bgPrimary, rounded corners=4pt,
    minimum width=2.2cm, minimum height=1.0cm,
    font=\sffamily\small, text=textMain, line width=0.6pt, align=center,
  },
  novelmodule/.style={
    draw=borderAccent, fill=bgAccent, rounded corners=4pt,
    minimum width=2.2cm, minimum height=1.0cm,
    font=\sffamily\small\bfseries, text=textMain, line width=1.1pt, align=center,
  },
  iobox/.style={
    draw=borderPrimary, fill=bgInput, rounded corners=3pt,
    minimum width=1.8cm, minimum height=0.8cm,
    font=\sffamily\small, text=textMain, line width=0.5pt, align=center,
  },
  stdarrow/.style={
    -{Stealth[length=5pt, width=4pt]}, line width=0.7pt, color=arrowColor,
  },
  arrowlabel/.style={font=\scriptsize\sffamily, text=textLight},
}


\ificlr
  \newcommand{\iclrfigwidth}{0.62\textwidth}
  \makeatletter
  \AtBeginDocument{%
    \let\iclr@origfigure\figure
    \let\iclr@origendfigure\endfigure
    \renewenvironment{figure}[1][tbp]{%
      \iclr@origfigure[#1]\centering\begin{minipage}{\iclrfigwidth}}{%
      \end{minipage}\iclr@origendfigure}%
  }
  \makeatother
\fi

